How Optimal is Greedy Decoding for Extractive Question Answering?

Fine-tuned language models use greedy decoding to answer reading comprehension questions with relative success. However, this approach does not ensure that the answer is a span in the given passage, nor does it guarantee that it is the most probable one. Does greedy decoding actually perform worse than an algorithm that does adhere to these properties? To study the performance and optimality of greedy decoding, we present exact-extract, a decoding algorithm that efficiently finds the most probable answer span in the context. We compare the performance of T5 with both decoding algorithms on zero-shot and few-shot extractive question answering. When no training examples are available, exact-extract significantly outperforms greedy decoding. However, greedy decoding quickly converges towards the performance of exact-extract with the introduction of a few training examples, becoming more extractive and increasingly likelier to generate the most probable span as the training set grows. We also show that self-supervised training can bias the model towards extractive behavior, increasing performance in the zero-shot setting without resorting to annotated examples. Overall, our results suggest that pretrained language models are so good at adapting to extractive question answering, that it is often enough to fine-tune on a small training set for the greedy algorithm to emulate the optimal decoding strategy.

==> tab_t5_large_em.tex <==

\begin{table*}[h!]
\small
\centering
\begin{tabular}{llccccccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &
{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{9}{c}{\textbf{\#Examples}} \\
&  &
  {\textbf{0}} &
  {\textbf{16}} &
  {\textbf{32}} &
  {\textbf{64}} &
  {\textbf{128}} &
  {\textbf{256}} &
  {\textbf{512}} &
  {\textbf{1024}} &
  \textbf{All} \\ 
\midrule
\multirow{2}{*}{\textbf{SQuAD}} & \textit{Greedy} &   40.9 &   71.0 &   72.9 &   74.6 &   78.8 &   79.5 &   81.2 &   82.9 &   87.9 \\
           & \textit{Exact-Extract} &   \textbf{53.1} &   \textbf{73.9} &   \textbf{76.2} &   \textbf{77.3} &   \textbf{80.8} &   \textbf{81.6} &   \textbf{82.7} &   \textbf{83.9} &   \textbf{88.5} \\
\midrule
\multirow{2}{*}{\textbf{TriviaQA}} & \textit{Greedy} &   57.1 &   66.1 &   63.3 &   63.1 &   66.2 &   69.0 &   72.1 &   75.6 &   78.9 \\
           & \textit{Exact-Extract} &   \textbf{63.0} &   \textbf{70.2} &   \textbf{70.1} &   \textbf{70.6} &   \textbf{72.3} &   \textbf{73.1} &   \textbf{74.7} &   \textbf{76.4} &   \textbf{79.9} \\
\midrule
\multirow{2}{*}{\textbf{NaturalQs}} & \textit{Greedy} &   30.5 &   46.5 &   49.1 &   49.9 &   53.6 &   55.6 &   57.5 &   59.0 &   68.7 \\
           & \textit{Exact-Extract} &   \textbf{44.4} &   \textbf{51.4} &   \textbf{53.6} &   \textbf{54.8} &   \textbf{57.2} &   \textbf{58.3} &   \textbf{60.1} &   \textbf{61.2} &   \textbf{70.3} \\
\midrule
\multirow{2}{*}{\textbf{NewsQA}} & \textit{Greedy} &   14.7 &   27.6 &   28.9 &   29.2 &   32.3 &   35.5 &   39.4 &   44.6 &   55.0 \\
           & \textit{Exact-Extract} &   \textbf{26.2} &   \textbf{31.4} &   \textbf{33.2} &   \textbf{34.5} &   \textbf{37.1} &   \textbf{40.0} &   \textbf{42.8} &   \textbf{46.9} &   \textbf{56.8} \\
\midrule
\multirow{2}{*}{\textbf{SearchQA}} & \textit{Greedy} &   21.2 &   55.7 &   55.9 &   63.4 &   65.3 &   71.7 &   74.5 &   \textbf{77.2} &   \textbf{83.0} \\
           & \textit{Exact-Extract} &   \textbf{31.2} &   \textbf{57.8} &   \textbf{59.9} &   \textbf{65.5} &   \textbf{67.1} &   \textbf{72.8} &   \textbf{74.8} & 77.1 &   82.8 \\
\midrule
\multirow{2}{*}{\textbf{HotpotQA}} & \textit{Greedy} &   32.8 &   50.7 &   \textbf{54.6} &   \textbf{57.3} &   \textbf{58.8} &   \textbf{60.5} &   \textbf{61.5} &   \textbf{62.8} &   \textbf{67.3} \\
           & \textit{Exact-Extract} &   \textbf{40.1} &   \textbf{50.8} &   54.3 &   57.1 &   58.6 &   60.2 &   61.1 &   62.5 &   66.6 \\
\midrule
\multirow{2}{*}{\textbf{BioASQ}} & \textit{Greedy} &   43.5 &   \textbf{63.1} &   \textbf{66.4} &   \textbf{71.7} &   \textbf{79.0} &   \textbf{86.0} &   \textbf{88.9} &   \textbf{92.1} &     -- \\
           & \textit{Exact-Extract} &   \textbf{54.5} &   62.7 &   66.0 &   71.4 &   77.8 &   84.5 &   88.0 &   90.8 &     -- \\
\midrule
\multirow{2}{*}{\textbf{TextbookQA}} & \textit{Greedy} &   15.0 &   35.0 &   36.2 &   41.1 &   45.4 &   52.6 &   62.2 &   \textbf{66.2} &     -- \\
           & \textit{Exact-Extract} &   \textbf{29.5} &   \textbf{42.7} &   \textbf{44.5} &   \textbf{48.6} &   \textbf{50.4} &   \textbf{55.1} &   \textbf{63.0} &   66.0 &     -- \\
\bottomrule
\end{tabular}
\caption{Performance (Exact-Match) across all datasets and training set sizes of the few-shot QA benchmark, as well as the zero-shot setting (\textbf{0} examples, no fine-tuning), and the full-data setting (\textbf{all} examples) as in the 2019 MRQA Shared Task, containing an order of 100,000 training examples per dataset. \Or{not referenced at all in the paper; need to decide if to remove}}
\label{tab:em_t5_large}
\end{table*}
